ERIM: Secure, Efficient In-process Isolation with Memory Protection Keys (MPK)

Isolating sensitive state and data can increase the security and robustness of many applications. Examples include protecting cryptographic keys against exploits like OpenSSL's Heartbleed bug or protecting a language runtime from native libraries written in unsafe languages. When runtime references across isolation boundaries occur relatively infrequently, then conventional page-based hardware isolation can be used, because the cost of kernel- or hypervisor-mediated domain switching is tolerable. However, some applications, such as the isolation of cryptographic session keys in network-facing services, require very frequent domain switching. In such applications, the overhead of kernel- or hypervisor-mediated domain switching is prohibitive. In this paper, we present ERIM, a novel technique that provides hardware-enforced isolation with low overhead on x86 CPUs, even at high switching rates (ERIM's measured overhead is less than 1% for 100,000 switches per second). The key idea is to combine protection keys (MPKs), a feature recently added to x86 that allows protection domain switches in userspace, with binary inspection to prevent circumvention. We show that ERIM can be applied with little effort to new and existing applications, doesn't require compiler changes, can run on a stock Linux kernel, and has low runtime overhead even at high domain switching rates.

==> discussion.tex <==
\section{Discussion}


\peter{Should discuss here additional applications of \erim.}

\todo{AV: Discussion about security properties of MPK and how to
  improve it - e.g. by adding a jump to WRPKRU instruction, 
eliminating WRPKRU occurrences is not necessary any more}


==> relatedwork.tex <==
\section{Related Work}
\label{erim:sec:relatedwork}

\peter{Suggest to integrate this material in Section 2.}

Reference monitors~\cite{Anderson1972} mediate privileged access by
untrusted applications protecting data confidentiality and integrity,
by sandboxing the application or checks inserted into the applications
execution. All implementations share the important property of
protecting the reference monitor's code and state from corruption and
deploy isolation techniques shielding the reference
monitor. Least-privilege and privilege separation~\cite{Saltzer1975}
define the basis for today's reference monitor mechanisms in hardware
(\cite{flicker, INTELSGX, ARMTZ}), hypervisors (\cite{Barham2003,
Belay2012}), operating systems (\cite{Watson2010, Elnikety2016}) or
applications (\cite{sfi, pittsfield, Ford2008, nativeclient,
Chen2016}). Two recent surveys
\cite{sokwarinmemory, Shu2016} show viable attacks and possible counter
measures to protect against data confidentiality and integrity
violations. Furthermore their interception granularity varies from a
separate guest OS (\cite{Barham2003}), a single application
(\cite{Belay2012, Bittau2008, Watson2010}) or application components
(\cite{sfi, flicker, Litton2016, pittsfield, Ford2008, nativeclient,
Chen2016, Zhou2014}). Intercepting at fine granularity offers
isolation across application components, whereas course-grain
interception isolates independent applications or components. Due to
its frequent invocations, fine-grained interception solutions require
isolation techniques with low overhead. \erim\ isolates
application components and intercepts fine-grained security relevant
events within the application, similarly to ARMlock~\cite{Zhou2014} or
SFI-based isolation~\cite{sfi, pittsfield, Ford2008,
nativeclient}. This is in contrast to techniques using OS process
boundaries (\cite{Litton2016}) or CPU privilege levels
(\cite{Belay2012, Barham2003}).

Shreds~\cite{Chen2016} monitors and protects security relevant
variables within applications. It requires annotations by the
programmer and a compiler pass to insert control switches. At runtime,
an isolated memory region is established and when a variable is used,
the application switches into the region. Using Shreds annotation and
compiler pass, \erim\ could be used for isolating code and data
into a separate protection region.

Aurasium~\cite{Xu2012} similarly to \erim\ places the
interception within the application's address space to dynamically
relink Android framework invocations and control access to private
user data. In contrast to \erim, Aurasium does not protect the
reference monitor's memory from accesses by malicious applications and
hence, may be circumvented by an attacker.

\textbf{Hardware-based reference monitors.}
Recent additions to Intel's~\cite{INTELSGX} and ARM's~\cite{ARMTZ} ISA
allow applications to execute a trusted part in a trusted execution engine (TEE).
Isolated from the remaining hypervisor, operating system or
applications, TEE's provide strong isolation and require
targeted implementations. Research systems use TEEs to reduce
the TCB (see Flicker~\cite{flicker}) needed to execute code
securely. Due to their strong isolation, TEE's do not allow
direct access to OS services like filesystem or network which limits
the usage due to overheads while crossing the isolation
boundary. \erim\ isolates application components, similar to Flicker,
while maintaining the programming model allowing access to OS
services.  

Haven~\cite{Baumann2015} and SCONE~\cite{Arnautov2016} provide a
systematic approach to run entire applications in TEEs while
providing OS services. This shields entire applications from their
environment instead of protecting a specific application
part. Security vulnerabilities existing in the unshielded application,
also exist in the shielded execution which attacks may use to violate
memory safety. As a result research is already looking at using memory
safety techniques~\cite{sgxbounds} in TEEs.

In addition to TEEs Intel also added support for bound checks
using Intel MPX and memory regions
with MPK~\cite{Intel2016}. Both techniques have been studied
for their effectiveness and adaptability in \cite{Koning2017,
Oleksenko2017}. Originally designed to enforce memory bounds on
application's data structure accesses, MPX efficiently isolates
memory, when dividing into few regions. Once the program uses more
regions, the internal bound registers need to access shadow copies
from main memory and stall executions. In addition MPX currently
allows only single-threaded applications. \cite{Koning2017} presents
memory isolation based on MPK to protect against accidental
memory leaks e.g. by bugs. \erim\ similarly uses MPK's
memory isolation to protect the reference monitor and targets a
stronger threat model allowing malicious attacks which requires
hardening MPK's isolation guarantees.

\textbf{Hypervisor/OS-based reference monitors.}
Today's processors provide several protection rings to isolate
hypervisors, OSes and application. Invented to provide efficient
virtualization of the underlying hardware, e.g.,
Xen~\cite{Barham2003}, Wedge~\cite{Bittau2008} and
Dune~\cite{Belay2012} isolate application components to run at
different ring levels and monitor OS resources.  

Similarly, OSes implement protection mechanisms like
Capsicum~\cite{Watson2010} monitoring an application's use
of OS resources. Light-weight contexts~\cite{Litton2016}
separate the address space, credentials and file identifiers from an
application process allowing applications to protect secrets in an
isolated memory address space. All these systems rely on special CPU
instructions to switch between regions which are costly. \erim\ on the
other hand switches within the same address space reducing the overall
switch overhead and allowing CPU caches to stay effective. In
addition \erim\ allows reference monitors access to the untrusted
application's memory which is not efficient for most of the above
systems.

Systems to automatically divide applications into different privilege
levels use OS process boundaries as protection~\cite{Brumley2004,
Kilpatrick2003}. Their utility is limited by the switching overhead
across processes to monitoring infrequent events like file descriptor
creations (open, fopen). In \erim\ the monitor similarly controls
OS service access to untrusted applications, while reducing the switch
overhead between monitor and application.

\textbf{Software-fault isolation (SFI).} 
\cite{sfi} introduces SFI, a technique to sandbox
untrusted applications and control access to OS services. Followed by
numerous papers advancing the guarantees, threat model, and
performance (\cite{Zhou2014, pittsfield, Ford2008, nativeclient}).
SFI sandboxes alter the binary before execution at 
compilation or by binary rewriting, or dynamically emulate
instructions to enforce memory isolation and restrict access to OS
services. \erim\ provides the framework to implement SFI as
described in section~\ref{erim:sec:usecases}. Instead of relying on a
compiler or emulator, \erim\ trusts the Intel CPU and its monitor to
enforce memory isolation.  

Recent systems~\cite{Ansel2011} adapt SFI to just-in-time compiled languages like JavaScript or C\#. This system isolates the application's execution from the language runtime. Their technique ports the binary code generator of V8 (JavaScript) and Mono (C\#) to generate NaCl restricted binary code. Similarly, \erim\ may isolate the application from the language runtime. Instead of generating NaCl restricted binary code, an \erim-protected code generator is only restricted not to generate a WRPKRU sequence. Excluding WRPKRU sequence from the binary code is simpler than the NaCl requirements which e.g. aligns instructions to 16 bytes and adds NOP padding.

\textbf{Inlined reference monitoring (IRM).}
In contrast to SFI which sandboxed the untrusted application,
IRM \cite{Erlingsson2000} includes security policy checks into the
untrusted application itself. These mechanisms insert during the
compilation stage checks before, e.g., memory accesses, jumps or
function returns and protect the execution from violating memory
confidentiality or integrity, control-flow integrity
(CFI) \cite{Abadi2005} or code-pointer integrity
(CPI) \cite{cpi}. CPI, e.g., still relies on confidentiality of its
state (pointer tables) and relies on ASLR in its 64-bit
implementation. \erim\ provides a framework for these mechanisms
to efficiently isolate their run-time state and perform necessary
checks.

\textbf{Memory hiding.} 
To avoid memory leaks, in-process memory isolation is used to protect
secret encryption keys or user's private data e.g. from attacks using
memory leaks. Hiding these secrets at random locations and restricting
pointer computations or constantly randomizing the layout of code has
been an active field in the past (\cite{Shacham2004,
Homescu2013}). Due to its probabilistic guarantees research has
consistently found attacks (\cite{Hund2013, Evans2015,
Oikonomopoulos2016, Goktacs2016}). \erim\ does not rely on
randomization, but has comparable performance.

Extended page tables hide secrets in execute-only pages by loading the
secret into CPU registers, computing the function and destroying the
contents of the register. Redactor~\cite{Crane2015} and
NEAR~\cite{Werner2016} hide code pointers in execute-only memory to
prevent code disclosure which is used by return-oriented programming
attacks. 

